DREAM: Deep Regret minimization with Advantage baselines and Model-free learning

We introduce DREAM, a deep reinforcement learning algorithm that finds optimal strategies in imperfect-information games with multiple agents. Formally, DREAM converges to a Nash Equilibrium in two-player zero-sum games and to an extensive-form coarse correlated equilibrium in all other games. Our primary innovation is an effective algorithm that, in contrast to other regret-based deep learning algorithms, does not require access to a perfect simulator of the game to achieve good performance. We show that DREAM empirically achieves state-of-the-art performance among model-free algorithms in popular benchmark games, and is even competitive with algorithms that do use a perfect simulator.

==> core/DONT_TOUCH_1.tex <==
\section{Review of Deep CFR and Single Deep CFR}
\label{sec:deepcfr}
Deep CFR~\cite{brown2019deep} approximates the behavior of tabular CFR from partial game tree traversals. For each CFR iteration~$t$, Deep CFR runs a constant $T$ external sampling traversals to collect samples of instantaneous regret and adds the data to a reservoir buffer $B^d_i$~\cite{reservoirSampling}, where agent~$i$ is the traverser. Deep CFR then trains a \textbf{value network}~$\hat{D}^t_i$ to predict the average regret (divided by external reach) for unseen infostate actions. $\hat{D}
^t_i$ is then used to approximate the policy $\pi^{t+1}_i$ for agent~$i$ like tabular CFR would produce given $R^t_i$. More data is collected by sampling based on this policy, and the process repeats until convergence.

Specifically, on each iteration $T$, the algorithm fits a value network $\hat{D}^T_i$ for one agent~$i$ to approximate \textbf{advantages} defined as \(D^T_i(s_i,a_i) = \frac{R^T_{i}(s_i, a_i)}{\sum_{t=1}^T (x_{-i}^{\pi^t}(s_i))}\). Deep CFR divides $R^T_i(s_i, a_i)$ by \(\sum_{t=1}^T (x_{-i}^{\pi^t}(s_i))\) to erase the difference in magnitude arising from highly varying realisation probabilities across infostates, which makes the data easier for the value network to approximate. This division does not change the policy output by Equation~\ref{eq:vanCFRiterStrat} since every action in an infostate is divided by the same value.

In cases where Deep CFR predicts non-positive advantage for all infostate actions, it chooses the action with the highest advantage rather than a uniform random policy as vanilla CFR would do.

Since it is the \emph{average} policy that converges to a Nash equilibrium in CFR, not the final strategy, Deep CFR trains a second neural network~$\hat{S}$ to approximate the average policy played over all iterations. Data for $\hat{S}_i$ is stored in a separate reservoir buffer $B^s_i$ and collected during the same traversals that data for $B^v_i$ is being collected on.

Single Deep CFR (SD-CFR) is a modification of Deep CFR that instead stores all value networks from each CFR iteration to disk and mimics the average policy exactly during play by sampling one of them and using its policy for the entire game. This is mathematically equivalent to sampling actions from the average policy. SD-CFR eliminates the approximation error in Deep CFR resulting from training a network to predict the average policy, at the minor cost of using extra disk space to store the models from each CFR iteration (or a random sample of CFR iterations).

==> core/DONT_TOUCH_2.tex <==


\section{Review of Monte-Carlo CFR with Baselines}

\subsection{Monte Carlo CFR (MC-CFR)}
Monte Carlo CFR (MC-CFR) is a framework that allows CFR to only update regrets on part of the tree for a single agent, called the \textbf{traverser}. Two variants relevant to our work are \textbf{External Sampling (ES)} and \textbf{Outcome Sampling (OS)}~\cite{lanctot2009monte}. In OS, regrets are updated for the traverser only along a single trajectory (i.e., a single action is sampled for each agent at each decision point, and a single outcome is sampled from $\mathcal{T}$). In ES, a single action is sampled for each non-traverser agent and a single outcome is sampled from $\mathcal{T}$, but every traverser action is explored. When agent~$i$ is the traverser in ES or OS, all other agents sample actions according to $\pi_{-i}$. In OS, we use a sampling policy~$\xi^t_i(s_i)$ profile rather than~$\pi^t$ to choose actions during play. $\xi^t_i(s_i)$ is defined separately for the traverser~$i$ and any other agent~$j$
\begin{equation} \label{eq:DREAMSamPoli}
\xi^{t}_i(s_i, a_i) = \epsilon\frac{1}{|\mathcal{A}_i(s_i)|} + (1-\epsilon)\pi^t_i(s_i, a_i)
\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }
\xi^{t}_{j}(s_j, a_j) = \pi^{t}_{j}(s_j, a_j)
\end{equation}
For a thorough and more general description of MC-CFR see~\cite{lanctot2009monte}.

\subsection{Variance-Reduced Outcome Sampling with Baselines}
ES typically produces lower-variance estimates of expected values than OS. Variance-reduced MC-CFR (VR-MC-CFR) is a method to reduce variance in MC-CFR and is particularly helpful for OS~\cite{schmid2019variance,davis2019low}. Given that OS ultimately reaches a terminal history $z$, the \textbf{baseline-adjusted sampled expected value} in history $h$ is
\begin{equation} \label{eq:VRMC-CFRva}
    \Tilde{v}_{i}^{\pi^t}(s_i(h),a_i) =
    \Tilde{v}_{i}^{\pi^t}(h,a_i) =
    \begin{cases}
        b_{i}(h, a_i) + \frac{\sum_{h'}\{p(h' | \mathcal{T}(h,a_i,\pi_{-i}^t))\Tilde{v}_{i}^{\pi^t}(h')\} - b_i(h,a_i)}{\xi_i^t(h,a_i)} & \text{if } (h, a_i) \sqsubset z \\
        
        b_i(h, a_i) & \text{otherwise}
    \end{cases}
\end{equation}
and 
\begin{equation} \label{eq:VRMC-CFRv}
    \Tilde{v}_{i}^{\pi^t}(s_i(h)) =
    \Tilde{v}_{i}^{\pi^t}(h) =
    \begin{cases}
        \mathcal{R}_i(h) & \text{if } h = z \\
        \sum_{a_i \in \mathcal{A}_i(h)} \pi_i^t(h,a_i) \Tilde{v}_{i}^{\pi^t}(h,a_i) & \text{otherwise} \\
    \end{cases}
\end{equation}
where $b$ is called the baseline, a user-defined scalar function that ideally is closely correlated with $v$. Common choices in the tabular setting are a running average across visits to any given history, and domain-specific estimates of $v$~\cite{schmid2019variance,davis2019low}.
\label{sec:vrMC-CFR}









\subsection{Variance-Reduced Outcome Sampling with Baselines}
\label{sec:vrMC-CFR}
ES typically produces lower-variance estimates of expected values than OS. Variance-reduced MC-CFR (VR-MC-CFR) is a method to reduce variance in MC-CFR and is particularly helpful for OS~\cite{schmid2019variance,davis2019low}. Given that OS ultimately reaches a terminal history $z$, the \textbf{baseline-adjusted sampled expected value} in history $h$ where action $a_i'$ is played leading to $h'$ is
\begin{equation} \label{eq:VRMC-CFRva}
    \Tilde{v}_{i}^{\pi^t}(s_i(h),a_i|z) =
    \Tilde{v}_{i}^{\pi^t}(h,a_i|z) =
    \begin{cases}
        b_{i}(s_i(h), a_i) + \frac{\Tilde{v}_{i}^{\pi^t}(h'|z) - b_i(s_i(h),a_i)}{\xi_i^t(s_i(h),a_i)} & \text{if } a_i = a_i' \\
        
        b_i(s_i(h), a_i) & \text{otherwise}
    \end{cases}
\end{equation}
and 
\begin{equation} \label{eq:VRMC-CFRv}
    \Tilde{v}_{i}^{\pi^t}(s_i(h)|z) =
    \Tilde{v}_{i}^{\pi^t}(h|z) =
    \begin{cases}
        \mathcal{R}_i(h) & \text{if } h = z \\
        \sum_{a_i \in \mathcal{A}_i(h)} \pi_i^t(s_i(h),a_i) \Tilde{v}_{i}^{\pi^t}(h,a_i) & \text{otherwise} \\
    \end{cases}
\end{equation}
where $b$ is called the baseline, a user-defined scalar function that ideally is closely correlated with $v$. Common choices in the tabular setting are a running average across visits to any given history, and domain-specific estimates of $v$~\cite{schmid2019variance,davis2019low}.


==> core/D_MCCFR.tex <==
\section{Review of Monte Carlo CFR (MC-CFR)} \label{app:MC-CFR}
Monte Carlo CFR (MC-CFR) is a framework that allows CFR to only traverse the parts of the game tree on each iteration. Two variants relevant to our work are \textbf{External Sampling (ES)} and \textbf{Outcome Sampling (OS)}~\cite{lanctot2009monte}. On an ES traversal, the traversing agent~$i$ follows all legal actions, but $-i$ and  $chance$ sample only one action.
The estimated EV for external sampling is defined recursively as
\begin{equation} \label{eq:MC-CFRcfv}
    \Tilde{v}_{i, ES}^{\pi^t}(h) =
    \begin{cases}
       \mathcal{R}(h)  & \text{if } h \text{ is terminal} \\
      \frac{1}{|\mathcal{A}_i(s)|} \sum_{a = (a_i = \in \mathcal{A}_i(s), a_{-i} \sim \mathcal{A}_{-i}(s))} (\mathcal{R}(h,a) + \pi_i^t(h,a) \Tilde{v}_{i, ES}^{\pi^t} (h \to a))          & \text{otherwise} \\
    \end{cases}
\end{equation}
and for $s_i = s_i(h)$, we approximate $\Tilde{v}_{i, OS}^{\pi^t}(s_i) = \Tilde{v}_{i, OS}^{\pi^t}(h)$.

OS samples only one action for every agent, meaning it traverses single trajectories without branching. Agent $i$ follows a sampling policy $\xi_i$ that, like any policy maps infostates $s$ to probabilities for actions in $\mathcal{A}_i(s_i)$. All other agent follow their $\pi^t_-i$ as determined by equation \ref{eq:vanCFRiterStrat}. Formally, the estimated EV for outcome sampling is defined recursively as

\begin{equation} \label{eq:MC-CFRcfv}
    \Tilde{v}_{i, OS}^{\pi^t}(h) =
    \begin{cases}
       \mathcal{R}_i(h)  & \text{if } h \text{ is terminal} \\
       \mathcal{R}_i(h)(h \to a) + \pi^t(h,a)\frac{\Tilde{v}_{i, OS}^{\pi^t} (h \to a}{\xi^t(h,a)})         & \text{if } s \to a \sqsubseteq h \text{, where } a \sim \xi^t \\
        0 & \text{otherwise} \\
    \end{cases}
\end{equation}
\(\)
and for $s_i = s_i(h)$, we approximate $\Tilde{v}_{i, OS}^{\pi^t}(s_i) = \Tilde{v}_{i, OS}^{\pi^t}(h)$.
